Cellular structures using $\textbf{U}_q$-tilting modules

We use the theory of $\textbf{U}_q$-tilting modules to construct cellular bases for centralizer algebras. Our methods are quite general and work for any quantum group $\textbf{U}_q$ attached to a Cartan matrix and include the non-semisimple cases for $q$ being a root of unity and ground fields of positive characteristic. Our approach also generalizes to certain categories containing infinite-dimensional modules. As applications, we give a new semisimplicty criterion for centralizer algebras, and recover the cellularity of several known algebras (with partially new cellular bases) which all fit into our general setup.

==> res/tilting.tex <==
In the present section we recall a few facts from the theory of $\Uq$-tilting modules.
In the semi-simple case all 
$\Uq$-modules in $\Mod{\Uq}$ are $\Uq$-tilting modules. 
Hence, the theory of $\Uq$-tilting modules is kind 
of redundant in this case.
In the non semi-simple case however the 
theory of $\Uq$-tilting modules is extremely rich and a source of neat combinatorics.
For brevity, we only provide proofs 
if we need the arguments of the proofs in what follows. For more details see for 
example~\cite{don1} and for arguments 
adopted to precisely our situation see~\cite{astproofs}.




\subsection{\texorpdfstring{$\Uq$}{Uq}-modules with a \texorpdfstring{$\Delta_q$}{Deltaq}- and a \texorpdfstring{$\nabla_q$}{nablaq}-filtration}\label{sub-tiltmod}

Recall that $\Nl$ has a simple socle and $\Dl$ has a simple head, both isomorphic to $\Ll$.
Thus, there is an (up to scalars) 
unique $\Uq$-homomorphism
\begin{equation}\label{eq-uniquemap}
c^{\lambda}\colon \Dl\to \Nl
\end{equation}
which sends the head to the socle. To see this, note that we have, by 
Frobenius reciprocity from~\eqref{eq-frob} (to be more precise, the $q$-version of 
it which can be found in~\cite[Proposition~2.12]{apw}),
\[
\Hom_{\Uq}(\Dl,\Nl)\cong\Hom_{\Uq^-\Uq^0}(\Dl,\K_{\lambda})
\]
which gives $\dim(\Hom_{\Uq}(\Dl,\Nl))=1$, since, by construction, $\Dl_{\lambda}\cong\K$.


This gives us the following (if $\Char(\K)>0$, then we have to 
enlarge the category $\Mod{\Uq}$ by non-necessarily finite-dimensional 
$\Uq$-modules to have enough injectives such that the 
$\Exti$-functors make sense by using $q$-analogous 
arguments as in~\cite[Part~I, Chapter~3]{jarag}).


\begin{thm}(\textbf{Ext-vanishing})\label{thm-extfunctor}
We have for all $\lambda,\mu\in X^+$ that
\[
\Exti(\Dl,\Nm)\cong\begin{cases}\K c^{\lambda},&\text{if }i=0\text{ and }\lambda=\mu,\\
0,&\text{else}.\end{cases}\hspace{3.3cm}
\raisebox{-0.25cm}{\makeqed}
\hspace{-3.3cm}
\]
\end{thm}
\begin{proof}
Similar to the modular analogon treated 
in~\cite[Part~2, Chapter~H.15]{jarag} 
(a proof in our notation can be found in~\cite{astproofs}).
\end{proof}


\begin{defn}(\textbf{$\Delta_q$- and $\nabla_q$-filtration})\label{defn-filt}
We say that a $\Uq$-module $M$ has a $\Delta_q$\textit{-filtration} 
if there exists some $k\in\N$ and 
a descending sequence of $\Uq$-submodules
\[
M=M_{0}\supset M_1\supset\cdots\supset M_{k^{\prime}}\supset\dots\supset M_{k-1}\supset M_k=0,
\]
such that for all $k^{\prime}=0,\dots,k-1$ 
we have $M_{k^{\prime}}/M_{k^{\prime}+1}\cong \Delta_q(\lambda_{k^{\prime}})$ 
for some $\lambda_{k^{\prime}}\in X^+$.

 
A $\nabla_q$\textit{-filtration} is defined similarly, 
but using $\nabla_q(\lambda)$ instead of $\Delta_q(\lambda)$ and 
an ascending sequence of $\Uq$-submodules, that is,
\[
0=M_{0}\subset M_1\subset\cdots\subset M_{k^{\prime}}\subset\dots\subset M_{k-1}\subset M_k=M,
\]
such that for all $k^{\prime}=0,\dots,k-1$ we have 
$M_{k^{\prime}+1}/M_{k^{\prime}}\cong \nabla_q(\lambda_{k^{\prime}})$ for some $\lambda_{k^{\prime}}\in X^+$.
\end{defn}


Clearly a 
$\Uq$-module $M$ has a $\Delta_q$-filtration iff its dual $\cal{D}(M)$ has a 
$\nabla_q$-filtration.



\begin{ex}\label{ex-filtration}
The simple $\Uq$-module $\Ll$ has a $\Delta_q$-filtration iff $\Ll\cong\Dl$. 
In that case we have also $\Ll\cong\Nl$ and thus, $\Ll$ has a 
$\nabla_q$-filtration as well.
\end{ex}



A corollary of the Ext-vanishing theorem is the following.


\begin{cor}\label{cor-extfunctor}
Let $M,N\in\Mod{\Uq}$ and $\lambda\in X^+$. Assume that 
$M$ has a $\Delta_q$-filtration and $N$ has a $\nabla_q$-filtration.
\begin{enumerate}[label=(\alph*)]
\item We have $\dim(\Hom_{\Uq}(M,\Nl))=(M:\Dl)=|\{k^{\prime}\mid\lambda_{k^{\prime}}=\lambda\}|$.
\item We have $\dim(\Hom_{\Uq}(\Dl,N))=(N:\Nl)=|\{k^{\prime}\mid\lambda_{k^{\prime}}=\lambda\}|$.
\end{enumerate}
Here the $\Uq$-weights $\lambda_{k^{\prime}}$ are as in Definition~\ref{defn-filt}.
In particular, the multiplicities $(M:\Dl)$ and $(N:\Nl)$ 
are independent of the choice of filtration.\makeqed
\end{cor}

Note that the proof of Corollary~\ref{cor-extfunctor} below gives 
a method to find and construct bases of $\Hom_{\Uq}(M,\Nl)$ and 
$\Hom_{\Uq}(\Dl,N)$ respectively.


\begin{proof}
Let $k$ be the length of the $\Delta_q$-filtration of $M$. If $k=1$, then
\begin{equation}\label{eq-additive}
\dim(\Hom_{\Uq}(M,\Nl))=(M:\Dl)
\end{equation} 
follows from the uniqueness of $c^{\lambda}$ from~\eqref{eq-uniquemap}.
Otherwise, we take the short exact sequence
\[
\xymatrix{
  0\ar[r] & M^{\prime}  \ar@{^{(}->}[r]    &  M  \ar@{->>}[r]  &  \Delta_q(\mu)\ar[r] & 0}
\]
for some $\mu\in X^+$. Since both sides of~\eqref{eq-additive} are additive with 
respect to short exact sequences by Theorem~\ref{thm-extfunctor}, the claim in (a) follows by induction.
Similarly for (b) by duality.
\end{proof}



In fact, following Donkin~\cite{don} who obtained the 
result below in the modular case, we can state two useful consequences of 
the Ext-vanishing theorem.
These are very useful criteria to determine if given $\Uq$-modules $M$ or $N$ have 
a $\Delta_q$- or $\nabla_q$-filtration respectively.


\begin{prop}(\textbf{Ext-criteria})\label{prop-extfunctor2}
Let $M,N\in \Mod{\Uq}$. Then the following are equivalent.

\begin{enumerate}[label=(\alph*)]
\item The $\Uq$-module $M$ has a $\Delta_q$-filtration
(respectively $N$ has a $\nabla_q$-filtration).
\item We have $\Exti(M,\Nl)=0$ 
(respectively $\Exti(\Dl,N)=0$)
for all $\lambda\in X^+$ and all $i>0$.
\item We have $\Extii(M,\Nl)=0$ 
(respectively $\Extii(\Dl,N)=0$)
for all $\lambda\in X^+$.\makeqed
\end{enumerate}
\end{prop}
\begin{proof}
As in~\cite[Proposition~II.4.16]{jarag}. 
A proof in our notation can be found in~\cite{astproofs}.
\end{proof}


\begin{ex}\label{ex-nonsplit}
Let us come back to our favorite example, i.e. $q$ being a 
complex, primitive 
third root of unity for $\Uq(\sll{2})$. The simple $\Uq$-module 
$L_q(3)$ does neither have a $\Delta_q$- nor a 
$\nabla_q$-filtration (compare 
Example~\ref{ex-sl2weylnext} with Example~\ref{ex-filtration}). 
This can also be seen 
with Proposition~\ref{prop-extfunctor2}, 
because $\Ext^1_{\Uq}(L_q(3),L_q(1))$ is not trivial: by 
Example~\ref{ex-sl2weylnext} from above 
we 
have $\Delta_q(1)\cong L_q(1)\cong\nabla_q(1)$, but
\[
\xymatrix{
  0\ar[r] & L_q(1)  \ar@{^{(}->}[r]    &  \Delta_q(3)  \ar@{->>}[r]  &  L_q(3)\ar[r] & 0}
\]
does not split. Analogously, $\Ext^1_{\Uq}(L_q(1),L_q(3))\neq 0$ by duality.
\end{ex}


\subsection{\texorpdfstring{$\Uq$}{Uq}-tilting modules}\label{sub-tiltmodprop}


Following Donkin~\cite{don}, we are now ready to define the 
\textit{category of} $\Uq$\textit{-tilting modules} that we denote by $\T$. This 
category is our main object of study.


\begin{defn}(\textbf{Category of $\Uq$-tilting modules})\label{defn-tiltcat}
The category $\T$ is the full subcategory 
of $\Mod{\Uq}$ whose objects are all $\Uq$\textit{-tilting modules}, 
that is, $\Uq$-modules $T$ which have both, a 
$\Delta_q$- and a $\nabla_q$-filtration.
\end{defn}



From Proposition~\ref{prop-extfunctor2} we obtain directly an important statement.


\begin{cor}\label{cor-tiltingext1}
Let $T\in\Mod{\Uq}$. Then
\[
T\in\T\quad\text{iff}\quad\Extii(T,\Nl)=0=\Extii(\Dl,T)\quad\text{for all }\lambda\in X^+.
\]
Moreover, the corresponding higher Ext-groups vanish as well.\qedmake
\end{cor}


Recall the contravariant, character preserving 
functor $\cal{D}\colon \Mod{\Uq}\to\Mod{\Uq}$ from~\eqref{eq-duality}. 
Clearly, by Corollary~\ref{cor-tiltingext1}, 
$T\in\T$ iff $\cal{D}(T)\in\T$. Thus, $\cal{D}(\cdot)$ restricts to a functor 
$\cal{D}\colon \T\to\T$. In fact, we show below in Corollary~\ref{cor-tiltingext3}, 
that the functor $\cal{D}(\cdot)$ restricts to (a functor isomorphic to) 
the identity functor on objects of $\T$.

\begin{ex}\label{ex-tilting}
The $\Ll$ are $\Uq$-tilting modules iff $\Dl\cong\Ll\cong\Nl$.



Coming back to our favourite example, that is the case $\fg=\sll{2}$ and 
$q$ is a complex, primitive third root of unity: 
a direct computation using similar reasoning as in 
Example~\ref{ex-sl2weylnext} (that is, the appearance of some 
actions equals zero as in~\eqref{eq-example2}) shows that $L_q(i)$ is a 
$\Uq$-tilting module iff $i=0,1$ or $i\equiv -1\;\mathrm{mod}\;3$.
More general: if $q$ is a complex, primitive $l$-th root of unity, then 
$L_q(i)$ is a 
$\Uq$-tilting module iff $i=0,\dots,l-1$ or $i\equiv -1\;\mathrm{mod}\;l$.
\end{ex}


\begin{prop}\label{prop-prop}
$\T$ is a Krull-Schmidt category, closed under 
duality $\cal{D}(\cdot)$ and under finite direct sums. 
Furthermore, $\T$ is closed under finite tensor products.\makeqed
\end{prop}


\begin{proof}
That $\T$ is a Krull-Schmidt is immediate. 
By Corollary~\ref{cor-tiltingext1} we see that 
$\T$ is closed under 
duality $\cal{D}(\cdot)$ and 
under finite direct sums.
That $\T$ is closed under finite tensor products is 
non-trivial
and a proof can be found in~\cite[Theorem~3.3]{par} 
(and a proof of a less general version sufficient for most 
of our purposes in~\cite{astproofs}).
\end{proof}



The 
indecomposable $\Uq$-modules in $\T$, that we denote by $\Tl$, are 
indexed by the dominant (integral) $\Uq$-weights $\lambda\in X^+$ 
(see Proposition~\ref{prop-tiltingclass} below).
The
$\Uq$-tilting module $\Tl$ is determined by the 
property that it is indecomposable with $\lambda$ as its unique maximal 
weight. Then $\lambda$ appears in fact with multiplicity $1$.


The following classification is, in the modular 
case, due to Ringel~\cite{ring} and Donkin~\cite{don}.


\begin{prop}(\textbf{Classification of the indecomposable $\Uq$-tilting modules})\label{prop-tiltingclass}
For each $\lambda\in X^+$ there exists an indecomposable  
$\Uq$-tilting module, that we denote by $\Tl$, with $\Uq$-weight spaces 
$\Tl_{\mu}=0$ unless $\mu\leq\lambda$. Moreover, $\Tl_{\lambda}\cong\K$.
In addition, given any indecomposable $\Uq$-tilting module $T\in\T$, then there exists 
$\lambda\in X^+$ such that $T\cong \Tl$.


Thus, the $\Tl$'s form a complete set of non-isomorphic indecomposables of $\T$ 
and all indecomposable $\Uq$-tilting modules $\Tl$ are uniquely 
determined by their maximal weight $\lambda\in X^+$, that is,
\[
\{\text{indecomposable }\Uq\text{-tilting modules}\}\stackrel{1:1}{\longleftrightarrow} X^+.
\hspace{3.7cm}
\makeqed
\hspace{-3.7cm}
\]
\end{prop}


\begin{proof}
Analogously to~\cite[Lemma~II.E.3 and Proposition~II.E.6]{jarag} and left to the reader.  
We only point out that one uses the $q$-version of 
the Frobenius reciprocity from~\eqref{eq-frob}. A detailed proof in our notation 
can be found in~\cite{astproofs}.
\end{proof}


\begin{rem}\label{rem-new}
For a fixed $\lambda\in X^+$ we have $\Uq$-homomorphisms
\[
\begin{gathered}
\xymatrix{
  \Dl  \ar@{^{(}->}[r]^{\iota^{\lambda}}    &  \Tl  \ar@{->>}[r]^{\pi^{\lambda}}  &  \Nl
}
\end{gathered}
\]
where $\iota^{\lambda}$ is the inclusion of the first 
$\Uq$-submodule in a $\Delta_q$-filtration of 
$\Tl$ and $\pi^{\lambda}$ is the surjection 
onto the last quotient in a $\nabla_q$-filtration of 
$\Tl$. Note that these are only defined up 
to scalars and we fix scalars in the following such that
$\pi^{\lambda}\circ\iota^{\lambda}=c^{\lambda}$ (where $c^{\lambda}$ is 
again the $\Uq$-homomorphism from~\eqref{eq-uniquemap}).


Take any $\Uq$-tilting module $T\in\T$. 
An easy argument shows (see also 
the proof of Proposition~\ref{prop-extfunctor2} in~\cite{astproofs}) 
the following crucial fact:
\begin{equation}\label{eq-important}
\Extii(\Dl,T)\hspace*{-0.3ex}=\hspace*{-0.3ex}0\hspace*{-0.3ex}=\hspace*{-0.3ex}\Extii(T,\Nl)\Rightarrow \Extii(\mathrm{coker}(\iota^{\lambda}),T)\hspace*{-0.3ex}=\hspace*{-0.3ex}0\hspace*{-0.3ex}=\hspace*{-0.3ex}\Extii(T,\ker(\pi^{\lambda}))
\end{equation}
for all $\lambda\in X^+$.
\DT{Hence, we see that any $\Uq$-homomorphism $g\colon \Dl\to T$ 
extends to an $\Uq$-homomorphism $\overline{g}\colon \Tl\to T$ 
whereas any $\Uq$-homomorphism $f\colon T\to \Nl$ factors 
through $\Tl$ via $\overline{f}\colon T\to\Tl$.}
\end{rem}




\begin{cor}\label{cor-tiltingext3}
We have $\cal{D}(T)\cong T$ for $T\in\T$, that is, all 
$\Uq$-tilting modules $T$ are self-dual. In particular, we have for all $\lambda\in X^+$ that
\[
(T:\Dl)=\dim(\Hom_{\Uq}(T,\Nl))=\dim(\Hom_{\Uq}(\Dl,T))=(T:\Nl).
\hspace{1.025cm}
\makeqed
\hspace{-1.025cm}
\]
\end{cor}



\begin{proof}
By the Krull-Schmidt property it suffices to show the statement for the 
indecomposable $\Uq$-tilting modules $\Tl$. Since $\cal{D}$ preserves 
characters, we see that $\cal{D}(\Tl)$ has $\lambda$ as unique maximal weight, therefore 
$\cal{D}(\Tl)\cong \Tl$ by Proposition~\ref{prop-tiltingclass}.
Moreover, the leftmost and the rightmost equalities follow directly from 
Corollary~\ref{cor-extfunctor}.
Finally
\[
(\Tl:\Dl)=(\cal{D}(\Tl):\cal{D}(\Dl))=(\cal{D}(\Tl):\Nl)=(\Tl:\Nl)
\] 
by definition and $\cal{D}(\Tl)\cong \Tl$ from above, which settles also the middle equality.
\end{proof}



\begin{ex}\label{ex-sl2c}
Let us go back to the $\sll{2}$ case again. Then we obtain the 
family $(T_q(i))_{i\in\N}$ of indecomposable 
$\Uq$-tilting modules as follows. 


Start by setting 
$T_q(0)\cong\Delta_q(0)\cong L_q(0)\cong\nabla_q(0)$ and 
$T_q(1)\cong\Delta_q(1)\cong L_q(1)\cong\nabla_q(1)$. 
Then we denote by $m_0\in T_q(1)$ any eigenvector for $K$ with eigenvalue $q$. 
For each $i>1$ we define $T_q(i)$ to be the indecomposable summand of 
$T_q(1)^{\otimes i}$ which contains the vector 
$m_0\otimes\cdots\otimes m_0\in T_q(1)^{\otimes i}$.
The $\Uq(\sll{2})$-tilting module $T_q(1)^{\otimes i}$ 
is not indecomposable if $i>1$: by Proposition~\ref{prop-tiltingclass} we have 
$(T_q(1)^{\otimes i}:\Delta_q(i))=1$ and
\[
T_q(1)^{\otimes i}\cong T_q(i)\oplus\bigoplus_{k<i}T_q(k)^{\oplus \mathrm{mult}_k}\quad
\text{for some }\mathrm{mult}_k\in\N.
\]
In the case $l=3$, we have for instance 
$T_q(1)^{\otimes 2}\cong T_q(2)\oplus T_q(0)$
since the tensor product $T_q(1)\otimes T_q(1)$ looks as follows 
(abbreviation $m_{ij}=m_i\otimes m_j$):
\[
\begin{gathered}
\xymatrix{
 \otimes \ar@{.}[r]\ar@{.}[d]& m_1 \ar@<2pt>[r]^{1}\ar@(ul,ur)|{q^{-1}}  &  m_0  \ar@<2pt>[l]^1\ar@(ul,ur)|{q^{+1}}  \\
 m_1\ar@<2pt>[d]^{1}\ar@(ul,dl)|{q^{-1}} & m_{11} \ar@<2pt>[r]^{1}\ar@<2pt>[d]^{1}\ar@(ul,dl)|{q^{-2}}  &  m_{01}  \ar@<2pt>[l]^1\ar@<2pt>[d]^{1}\ar@{.}[dl]|{+}\ar@(ur,dr)|{q^{0}}  \\
 m_0\ar@<2pt>[u]^{1}\ar@(ul,dl)|{q^{+1}} & m_{10} \ar@<2pt>[r]^{1}\ar@<2pt>[u]^{1}\ar@(ul,dl)|{q^{0}}  &  m_{00}  \ar@<2pt>[l]^1\ar@<2pt>[u]^{1}\ar@(ur,dr)|{q^{+2}}  \\
}
\end{gathered}.
\] 
By construction, the indecomposable $\Uq(\sll{2})$-module 
$T_q(2)$ contains $m_{00}$ and therefore 
has to be the $\C$-span of $\{m_{00},q^{-1}m_{10}+m_{01},m_{11}\}$ as 
indicated above. The remaining summand
is the $1$-dimensional 
$\Uq$-tilting module $T_q(0)\cong L_q(0)$ from before.
\end{ex}


The following is interesting in its own right.
\begin{cor}\label{cor-thelast-really}
Let $\mu\in X^+$ be a minuscule $\Uq$-weight. Then 
$T=\Dm^{\otimes d}$ is a $\Uq$-tilting module for any $d\in\N$ and 
$\dim(\Endrr)$ is independent of the field $\K$ and of $q\in\K^{\ast}$
(and given by~\eqref{eq-dimhom}). 
In particular, this holds for
$\Delta_q(\omega_1)$ being the vector 
representation of $\Uq=\Uq(\fg)$ for $\fg$ of 
type $A$, $C$ or $D$.\makeqed
\end{cor}


\begin{proof}
Since $\mu\in X^+$ is minuscule: $\Dm\cong\Lm$ is a 
simple $\Uq$-tilting module for any field $\K$ and any $q\in\K^{\ast}$.
Thus, by Proposition~\ref{prop-prop} we see that $T$ is a $\Uq$-tilting module for any $d\in\N$. 
Hence, by Corollaries~\ref{cor-extfunctor} and~\ref{cor-tiltingext3}, 
we have $\dim(\Endrr)=\sum_{\lambda\in X^+}(T:\Dl)^2$.
Now use the fact that $\chi(\Dm)$ is as in the classical case 
which implies the statement.
\end{proof}



\subsection{The characters of indecomposable \texorpdfstring{$\Uq$}{Uq}-tilting modules}\label{sub-char}


In this subsection we describe how to compute 
$(\Tl:\Dm)$ 
for all $\lambda,\mu\in X^+$ (which can be done algorithmically 
in the case where $q$ is a 
complex, primitive $l$-th root of unity). 
As an application, we illustrate how to decompose tensor products 
of $\Uq$-tilting modules. This shows that, in principle, our cellular basis 
for endomorphism rings $\Endrr$ of $\Uq$-tilting modules $T$ 
(that we introduce in Section~\ref{sec-endorings}) can be made completely explicit.

Given an abelian category $\cal{AB}$, 
we denote its \textit{Grothendieck group} by
$K_0(\cal{AB})$ and its 
\textit{split Grothendieck group} by $K^{\oplus}_0(\cal{AB})$. 
We point out that the notation of the split Grothendieck group also makes sense 
for a given additive category $\cal{AD}$  
that satisfies the Krull-Schmidt property where we use the same notation
(we refer the reader unfamiliar with these and the 
notation we use to~\cite[Section~1.2]{mar}).




By Propositions~\ref{prop-semisimple2} 
and~\ref{prop-nonsemisimple}, a $\Z$-basis of the Grothendieck group
$K_0(\Mod{\Uq})$ is given by isomorphism 
classes $\{[\Dl]\mid \lambda\in X^+\}$.


On the other hand, $\T$ is not abelian (see Example~\ref{ex-tilting}), but 
additive and satisfies the Krull-Schmidt property. A $\Z$-basis of $K^{\oplus}_0(\T)$ 
is, by Proposition~\ref{prop-tiltingclass}, 
spanned by isomorphism 
classes $\{[\Tl]_{\oplus}\mid \lambda\in X^+\}$.


\DT{Since both $\Mod{\Uq}$ and $\T$} are closed under tensor products, 
$K_0(\Mod{\Uq})$ and $K^{\oplus}_0(\T)$ get an (in fact isomorphic) 
induced ring structure.


\begin{cor}\label{cor-grothen}
The inclusion of categories $\iota\colon \T\to\Mod{\Uq}$ induces an isomorphism
\[
[\iota]\colon K^{\oplus}_0(\T)\to K_0(\Mod{\Uq}),
\quad [\Tl]_{\oplus}\mapsto [\Tl],\quad \lambda\in X^+
\]
of rings.\makeqed
\end{cor}


\begin{proof}
The set $B=\{[\Tl]\mid\lambda\in X^+\}$ forms a $\Z$-basis of $K_0^{\oplus}(\T)$ 
by Proposition~\ref{prop-tiltingclass} and it is clear that $[\iota]$ is 
a well-defined ring homomorphism.


Moreover, we have
\begin{equation}\label{eq-grgr}
[\Tl]=[\Dl]+\sum_{\mu<\lambda\in X^+}(T_q(\mu):\Delta_q(\mu))[\Delta_q(\mu)]\in K_0(\Mod{\Uq})
\end{equation}
with $T_q(0)\cong \Delta_q(0)$ by Proposition~\ref{prop-tiltingclass}. Hence, $[\iota](B)$ is also 
a $\Z$-basis of $K_0(\Mod{\Uq})$ since the $\Dl$'s form a $\Z$-basis and the claim follows.
\end{proof}


Recall that $\Z[X]$ carries an action of 
the Weyl group $W$ associated to the Cartan datum (see below). Thus, we can look at the invariant part of this action, 
denoted by $\Z[X]^W$, which is known as \textit{Weyl's character ring}.


We obtain the following (known) categorification result.


\begin{cor}\label{cor-cat}
The tilting category $\T$ (naively) categorifies Weyl's character ring, that is,
\[
K^{\oplus}_0(\T)\cong \Z[X]^W\quad\text{as rings}.
\hspace{5.325cm}
\makeqed
\hspace{-5.325cm}
\]
\end{cor}


\begin{proof}
It is known that there is an 
isomorphism $K_0(\Mod{\fg})\stackrel{\cong}{\longrightarrow}\Z[X]^W$ given by 
sending finite-dimensional $\fg$-modules to their characters 
(which can be regarded as elements in $\Z[X]^W$).



Now the characters $\chi(\Dl)$ of the $\Dl$'s are (as mentioned 
below Example~\ref{ex-sl2weylnext}) the same as in the classical case.
Thus, we can adopt the isomorphism 
from $K_0(\Mod{\fg})$ to $\Z[X]^W$ from above (non-quantized!).
Details can, for example, be 
found in~\cite[Chapter~VIII, \S 7.7]{bour}.


Then the statement follows from Corollary~\ref{cor-grothen}.
\end{proof}



For each simple root $\alpha_i\in \Pi$ let $s_i$ be the reflection
\[
s_i(\lambda)=\lambda-\langle\lambda,\alpha_i^{\vee}\rangle\alpha_i,\quad\text{for }\lambda\in E,
\]
in the hyperplane $H_{\alpha_i^{\vee}}$ 
orthogonal to $\alpha_i$. These reflections $s_i$ generate a group $W$, called
\textit{Weyl group}, associated to our Cartan datum.


For any fixed $l\in\N$, the \textit{affine Weyl group} 
$W_l\cong W\ltimes l\Z\Pi$ is the group 
generated by the reflections $s_{\beta,r}$ in the \textit{affine hyperplanes}
$H_{\beta^{\vee},r}=\{x\in E\mid\langle x,\beta^{\vee}\rangle=lr\}$ 
for $\beta\in\Phi$ and $r\in\Z$. Note that, if $l=0$, then $W_0\cong W$.


For $\beta\in\Phi$ there exists $w\in W$ such 
that $\beta=w(\alpha_i)$ for some $i=1,\dots,n$. We set 
$l_{\beta}=l_i$ where $l_i=\frac{l}{\mathrm{gcd}(l,d_i)}$.
Using this, we have the \textit{dot-action} of $W_l$ 
on the $\Uq$-weight lattice $X$ via
\[
s_{\beta,r}.\lambda=s_{\beta}(\lambda+\rho)-\rho+l_{\beta}r\beta.
\]
Note that the case $l=1$ recovers the usual action of the affine Weyl group $W_1$ on $X$.


\begin{defn}(\textbf{Alcove combinatorics})\label{defn-fundalc}
The \textit{fundamental alcove} $\cal{A}_0$ is
\begin{equation}\label{eq-condition1}
\cal{A}_0=\{\lambda \in X\mid 0<\langle \lambda+\rho,
\alpha^{\vee}\rangle<l,\text{ for all }\alpha\in\Phi^+\}\subset X^+.
\end{equation}
Its \textit{closure} $\overline{\cal{A}}_0$ is given by
\begin{equation}\label{eq-condition2}
\overline{\cal{A}}_0=\{\lambda \in X\mid 0\leq\langle \lambda+\rho,
\alpha^{\vee}\rangle \leq l,\text{ for all }\alpha\in\Phi^+\}\subset X^+-\rho.
\end{equation}


The \textit{non-affine walls} of $\cal{A}_0$ are
\[
\check{\partial}\cal{A}^i_0=\overline{\cal{A}}_0\cap (H_{\alpha_i^{\vee},0}-\rho),
 i=1,\dots,n,\quad \check{\partial}\cal{A}_0=\bigcup_{i=1}^n \check{\partial}\cal{A}^i_0.
\]
The set
\[
\hat{\partial}\cal{A}_0=\overline{\cal{A}}_0\cap (H_{\alpha_0^{\vee},1}-\rho)
\]
is called the \textit{affine} wall of $\cal{A}_0$. Here $\alpha_0$ is the maximal short root. 
We call the union of all these walls the \textit{boundary} $\partial\cal{A}_0$ of $\cal{A}_0$.
More generally, an 
\textit{alcove} $\cal{A}$ is a connected component of
\[
E-\bigcup_{r\in\Z,\beta\in\Phi}(H_{\beta^{\vee},r}-\rho).
\]
We denote the set of alcoves by $\cal{AL}$.
\end{defn}

Note that the affine Weyl group $W_l$ acts simply transitively on $\cal{AL}$. Thus, we can 
associate $1\in W_l\mapsto \cal{A}(1)=\cal{A}_0\in\cal{AL}$ and in general 
$w\in W_l\mapsto \cal{A}(w)\in\cal{AL}$.


\begin{ex}\label{ex-alcove}
In the case $\fg=\sll{2}$ we have $\rho=\omega_1=1$. Consider for instance again $l=3$. Then 
$k\in\N=X^+$ is contained in the fundamental alcove $\cal{A}_0$ iff $0<k+1<3$.


Moreover, $-\rho\in\check{\partial}\cal{A}_0$ and $2\in\hat{\partial}\cal{A}_0$ 
are on the walls. Thus, $\overline{\cal{A}}_0$ can be visualized as
\[
\xy
(0,0)*{
\begin{tikzpicture}[scale=.75]
	\draw [very thick] (0,0.025) to (3,0.025);
	\node[green] at (0,0) {\tiny $\bullet$};
	\node[red] at (3,0) {\tiny $\bullet$};
	\node at (0,0.25) {\tiny $-\rho$};
	\node at (1,0.25) {\tiny $0$};
	\node at (2,0.25) {\tiny $1$};
	\node at (3,0.25) {\tiny $2$};
\end{tikzpicture}
};
\endxy
\]
where the affine wall on the right 
is indicated in red and the non-affine wall  on the left 
is indicated in green.
\end{ex}


\begin{ex}\label{ex-alcoveb}
Let us leave our running $\sll{2}$ example for a second and do another 
example which is graphically more interesting.


In the case $\fg=\sll{3}$ we have $\rho=\alpha_1+\alpha_2=\omega_1+\omega_2\in X^+$ 
and $\alpha_0=\alpha_1+\alpha_2$.
Now consider again $l=3$. The condition~\eqref{eq-condition1} means that $\cal{A}_0$ consists of
those $\lambda=\lambda_1\omega_1+\lambda_2\omega_2$ for which
\[
0<\langle \lambda_1\omega_1+\lambda_2\omega_2+\omega_1+\omega_2,\alpha_i^{\vee}\rangle<3\quad\text{for }i=1,2,0.
\]
Thus, $0<\lambda_1+1<3$, $0<\lambda_2+1<3$ and $0<\lambda_1+\lambda_2+2<3$.
Hence, only the $\Uq(\sll{3})$-weight $\lambda=(0,0)\in X^+$ is in $\cal{A}_0$.
In addition, we have by condition~\eqref{eq-condition2} that
\[
\check{\partial}\cal{A}_0=\{-\rho,-\omega_1,-\omega_2, \omega_1-\omega_2,\omega_2-\omega_1\},
\quad\quad
\hat{\partial}\cal{A}_0=\{\omega_1,\omega_2,2\omega_1-\omega_2,2\omega_2-\omega_1\}.
\]
Hence, $\overline{\cal{A}}_0$ can be visualized as (displayed without the $-\rho$ shift on the left)
\[
\xy
(0,0)*{
\begin{tikzpicture}[scale=.75]
	\draw [very thick,green] (0,0) to (-1,1.73);
	\draw [very thick,blue] (0,0) to (1,1.73);
	\draw [very thick,red] (-1,1.73) to (1,1.73);
	\draw [very thick, directed=1.0] (0,0) to (1.06,0.613);
	\draw [very thick, directed=1.0] (0,0) to (-1.06,0.613);
	\node at (0,1) {\tiny $(1,1)$};
	\node at (0,0) {\tiny $\bullet$};
	\node at (-0.33,0.57) {\tiny $\bullet$};
	\node at (0.33,0.57) {\tiny $\bullet$};
	\node at (-0.33,1.7) {\tiny $\bullet$};
	\node at (0.33,1.7) {\tiny $\bullet$};
	\node at (0,-0.25) {\tiny $0$};
	\node at (-0.65,0.57) {\tiny $\omega_2$};
	\node at (0.65,0.57) {\tiny $\omega_1$};
	\node at (-0.7,1.9) {\tiny $2\omega_2{+}\omega_1$};
	\node at (0.7,1.9) {\tiny $2\omega_1{+}\omega_2$};
	\node at (1.3,0.65) {\tiny $\alpha_1$};
	\node at (-1.3,0.65) {\tiny $\alpha_2$};
	\node at (-0.66,1.133) {\tiny $\bullet$};
	\node at (0.66,1.133) {\tiny $\bullet$};
	\node at (-1,1.7) {\tiny $\bullet$};
	\node at (1,1.7) {\tiny $\bullet$};
	\node at (1.05,1.133) {\tiny $2\omega_1$};
	\node at (-1.05,1.133) {\tiny $2\omega_2$};
	\node at (1.4,1.64) {\tiny $3\omega_1$};
	\node at (-1.4,1.64) {\tiny $3\omega_2$};
\end{tikzpicture}
};
\endxy
\quad\quad
\xy
(0,0)*{
\begin{tikzpicture}[scale=.75]
	\draw [very thick,green] (0,0) to (-1,1.73);
	\draw [very thick,blue] (0,0) to (1,1.73);
	\draw [very thick,red] (-1,1.73) to (1,1.73);
	\node at (0,1) {\tiny $(0,0)$};
	\node at (0,0) {\tiny $\bullet$};
	\node at (-0.33,0.57) {\tiny $\bullet$};
	\node at (0.33,0.57) {\tiny $\bullet$};
	\node at (-0.33,1.7) {\tiny $\bullet$};
	\node at (0.33,1.7) {\tiny $\bullet$};
	\node at (0,-0.25) {\tiny $-\rho$};
	\node at (-0.75,0.57) {\tiny $-\omega_1$};
	\node at (0.75,0.57) {\tiny $-\omega_2$};
	\node at (-0.33,1.9) {\tiny $\omega_2$};
	\node at (0.33,1.9) {\tiny $\omega_1$};
	\node at (-0.66,1.133) {\tiny $\bullet$};
	\node at (0.66,1.133) {\tiny $\bullet$};
	\node at (-1,1.7) {\tiny $\bullet$};
	\node at (1,1.7) {\tiny $\bullet$};
	\node at (1.325,1.133) {\tiny $\omega_1{-}\omega_2$};
	\node at (-1.3,1.133) {\tiny $\omega_2{-}\omega_1$};
	\node at (1.75,1.7) {\tiny $2\omega_1{-}\omega_2$};
	\node at (-1.75,1.7) {\tiny $2\omega_2{-}\omega_1$};
\end{tikzpicture}
};
\endxy
\]
where, as before, the affine wall at the top is indicated in red, the hyperplane 
orthogonal to $\alpha_1$ on the left in green and the hyperplane 
orthogonal to $\alpha_2$ on the right in blue.
\end{ex}



We say $\lambda\in X^+-\rho$ is \textit{linked} to $\mu\in X^+$ 
if there exists $w\in W_l$ such that $w.\lambda=\mu$. We note the following theorem, 
called \textit{the linkage principle}, where we, by 
convention, set $\Tl=\Dl=\Nl=\Ll=0$ for 
$\lambda\in\check{\partial}\cal{A}_0$.



\begin{thm}(\textbf{The linkage principle})\label{thm-link}
All composition factors of $\Tl$ have maximal weights $\mu$ linked to 
$\lambda$. Moreover, $\Tl$ is a simple $\Uq$-module if $\lambda\in\overline{\cal{A}}_0$.

If $\lambda$ is linked to an element of $\cal{A}_0$, then 
$\Tl$ is a simple $\Uq$-module iff $\lambda\in\cal{A}_0$.\makeqed
\end{thm}
\begin{proof}
This is a slight reformulation of~\cite[Corollaries~4.4 and~4.6]{an2}.
\end{proof}


The linkage principle gives us now a decomposition into a direct sum of categories
\[
\T\cong \bigoplus_{\lambda\in\cal{A}_0}\T_{\lambda}\oplus\bigoplus_{\lambda\in\partial\cal{A}_0}\T_{\lambda},
\]
where each $\T_{\lambda}$ consists of all $T\in\T$ whose indecomposable 
summands are all of the form $T_q(\mu)$ for $\mu\in X^+$ 
lying in the $W_l$-dot-orbit of $\lambda\in\cal{A}_0$ (or of $\lambda\in\partial\cal{A}_0$).
We call these categories \textit{blocks} to stress that they are 
homologically unconnected (although they might be decomposable). Moreover, if 
$\lambda\in\cal{A}_0$, then we call 
$\T_{\lambda}$ an \textit{$l$-regular} block, 
while the 
$\T_{\lambda}$'s with $\lambda\in\partial\cal{A}_0$ are 
called 
\textit{$l$-singular} blocks (we say for short just regular 
and singular blocks in what follows).


In fact, by Proposition~\ref{prop-tiltingclass}, the $\Uq$-weights labelling the 
indecomposable $\Uq$-tilting 
modules are only the dominant (integral) weights $\lambda\in X^+$.
Let $\cal{DC}=\{x\in E\mid \langle x,\beta^{\vee}\rangle\geq 0,\beta\in\Phi\}$. 
Then these 
$\Uq$-weights correspond blockwise precisely to the alcoves
\[
\cal{AL}^+=\cal{AL}\cap\cal{DC},
\]
contained in the dominant chamber $\cal{DC}$.
That is, they correspond to the set of coset representatives of minimal length in 
$\{wW_0\mid w\in W_1\}$. In formulas,
\begin{equation}\label{eq-translationweyl}
T_q(w.\lambda)\in \T_{\lambda}\leftrightsquigarrow \cal{A}(w)\in\cal{AL}^+\leftrightsquigarrow wW_0\subset W_1,
\end{equation}
for all $\lambda\in\cal{A}_0$.


\begin{ex}\label{ex-sl2alcoves}
In our pet example with $\fg=\sll{2}$ and $l=3$ we have, by Theorem~\ref{thm-link} and 
Example~\ref{ex-alcove} a block decomposition
\[
\T\cong \T_{-1}\oplus \T_{0}\oplus\T_{1}\oplus\T_2.
\]
The $W_l$-dot-orbit of $0\in \cal{A}_0$ respectively $1\in \cal{A}_0$
can be visualized as
\[
\xy
(0,0)*{
\begin{tikzpicture}[scale=.75]
\draw [very thick,red, ->] (1,0.25) to [out=30,in=180] (3,0.75) to [out=0,in=150] (5,0.25);
\draw [very thick,green, ->] (5,0.25) to [out=60,in=180] (6,0.75) to [out=0,in=120] (7,0.25);
\draw [very thick,red, ->] (7,0.25) to [out=30,in=180] (9,0.75) to [out=0,in=150] (11,0.25);
\draw [very thick,green, ->] (11,0.25) to [out=60,in=180] (12,0.75) to [out=0,in=120] (13,0.25);
\draw [very thick,red, ->] (13,0.25) to [out=30,in=180] (15,0.75) to [out=0,in=150] (17,0.25);
\draw [very thick,green, ->] (17,0.25) to [out=60,in=180] (18,0.75);
\draw [very thick,red, ->] (2,-0.25) to [out=300,in=180] (3,-0.75) to [out=0,in=240] (4,-0.25);
\draw [very thick,green, ->] (4,-0.25) to [out=330,in=180] (6,-0.75) to [out=0,in=210] (8,-0.25);
\draw [very thick,red, ->] (8,-0.25) to [out=300,in=180] (9,-0.75) to [out=0,in=240] (10,-0.25);
\draw [very thick,green, ->] (10,-0.25) to [out=330,in=180] (12,-0.75) to [out=0,in=210] (14,-0.25);
\draw [very thick,red, ->] (14,-0.25) to [out=300,in=180] (15,-0.75) to [out=0,in=240] (16,-0.25);
\draw [very thick,green, ->] (16,-0.25) to [out=330,in=180] (18,-0.75);
	\node[green] at (0,0) {\tiny $\bullet$};
	\node[red] at (3,0) {\tiny $\bullet$};
	\node[green] at (6,0) {\tiny $\bullet$};
	\node[red] at (9,0) {\tiny $\bullet$};
	\node[green] at (12,0) {\tiny $\bullet$};
	\node[red] at (15,0) {\tiny $\bullet$};
	\node[orange] at (1,0) {\tiny $0$};
	\node[orange] at (5,0) {\tiny $4$};
	\node[orange] at (7,0) {\tiny $6$};
	\node[orange] at (11,0) {\tiny $10$};
	\node[orange] at (13,0) {\tiny $12$};
	\node[magenta] at (2,0) {\tiny $1$};
	\node[magenta] at (4,0) {\tiny $3$};
	\node[magenta] at (8,0) {\tiny $7$};
	\node[magenta] at (10,0) {\tiny $9$};
	\node[magenta] at (14,0) {\tiny $13$};
	\node[magenta] at (16,0) {\tiny $\cdots$};
	\node[orange] at (17,0) {\tiny $\cdots$};,
	\node at (0,0.25) {\tiny $\text{dead end}$};
	\node at (3,0.25) {\tiny $r=1$};
	\node at (6,0.25) {\tiny $r=2$};
	\node at (9,0.25) {\tiny $r=3$};
	\node at (12,0.25) {\tiny $r=4$};
	\node at (15,0.25) {\tiny $r=5$};
\end{tikzpicture}
};
\endxy
\]
Compare also 
to~\cite[(2.4.1)]{at}.



It turns out that, for $\K=\C$, both singular blocks $\T_{-1}$ and $\T_{2}$ are semi-simple 
(in particular, these blocks 
decompose further), see Example~\ref{ex-sl2again} or~\cite[Lemma~2.25]{at}.
\end{ex}


\begin{ex}\label{ex-sl3alcoves}
In the $\sll{3}$ case with $l=3$ we have the block decomposition
\[
\T\cong \T_{-\rho}\oplus \T_{-\omega_2}\oplus\T_{-\omega_1}\oplus
\T_{\omega_1-\omega_2}\oplus\T_{\omega_2-\omega_1}\oplus
\T_{(0,0)}\oplus
\T_{2\omega_1-\omega_2}\oplus\T_{\omega_1}\oplus\T_{\omega_2}\oplus\T_{2\omega_2-\omega_1}
\]
(note that the singular blocks are not necessarily semi-simple anymore, even when $\K=\C$).


The $W_l$-dot-orbit in $\cal{AC}^+$ of the regular block $\T_{(0,0)}$
looks as follows.
\[
\xy
(0,0)*{
\begin{tikzpicture}[scale=.75]
	\draw [very thick,green] (0,0) to (-1,1.73);
	\draw [very thick,green] (-1,1.73) to (-2,3.464);
	\draw [very thick,green] (1,1.73) to (0,3.464);
	\draw [very thick,green] (1,1.73) to (1.1,1.52);
	\draw [very thick,green] (0,3.464) to (-1,5.20);
	\draw [very thick,green] (2,3.464) to (1,5.20);
	\draw [very thick,green] (2,3.464) to (2.1,3.25);
	\draw [very thick,green] (-2,3.464) to (-3,5.20);
	\draw [very thick,blue] (0,0) to (1,1.73);
	\draw [very thick,blue] (-1,1.73) to (0,3.464);
	\draw [very thick,blue] (-1,1.73) to (-1.1,1.52);
	\draw [very thick,blue] (1,1.73) to (2,3.464);
	\draw [very thick,blue] (-2,3.464) to (-1,5.20);
	\draw [very thick,blue] (-2,3.464) to (-2.1,3.25);
	\draw [very thick,blue] (0,3.464) to (1,5.20);
	\draw [very thick,blue] (2,3.464) to (3,5.20);
	\draw [very thick,red] (-1,1.73) to (1,1.73);
	\draw [very thick,red] (1,1.73) to (1.25,1.73);
	\draw [very thick,red] (-2,3.464) to (0,3.464);
	\draw [very thick,red] (0,3.464) to (2,3.464);
	\draw [very thick,red] (2,3.464) to (2.25,3.464);
	\draw [very thick,red] (-3,5.20) to (-1,5.20);
	\draw [very thick,red] (-1,5.20) to (1,5.20);
	\draw [very thick,red] (1,5.20) to (3,5.20);
	\draw [very thick,red] (3,5.20) to (3.25,5.20);
	\draw [very thick, directed=1.0] (0,0) to (1.06,0.613);
	\draw [very thick, directed=1.0] (0,0) to (-1.06,0.613);
	\node at (-2.5,6) {\tiny $\vdots$};
	\node at (-1.5,6) {\tiny $\vdots$};
	\node at (-0.5,6) {\tiny $\vdots$};
	\node at (0.5,6) {\tiny $\vdots$};
	\node at (1.5,6) {\tiny $\vdots$};
	\node at (2.5,6) {\tiny $\vdots$};
	\node at (1.75,1.73) {\tiny $r=1$};
	\node at (2.75,3.464) {\tiny $r=2$};
	\node at (3.75,5.20) {\tiny $r=3$};
	\node at (-1.3,1.32) {\tiny $r=1$};
	\node at (-2.3,3.05) {\tiny $r=2$};
	\node at (1.3,1.32) {\tiny $r=1$};
	\node at (2.3,3.05) {\tiny $r=2$};
	\node at (1.3,0.65) {\tiny $\alpha_1$};
	\node at (-1.3,0.65) {\tiny $\alpha_2$};
	\end{tikzpicture}
};
\endxy
\rightsquigarrow
\xy
(0,0)*{
\begin{tikzpicture}[scale=.75]
	\draw [very thick,green] (0,0) to (-1,1.73);
	\draw [very thick,green] (-1,1.73) to (0,3.464);
	\draw [very thick,green] (0,3.464) to (2,3.464);
	\draw [very thick,green] (0,3.464) to (-1,5.20);
	\draw [very thick,green] (2,3.464) to (3,5.20);
	\draw [very thick,green] (-3,5.20) to (-1,5.20);
	\draw [very thick,blue] (0,0) to (1,1.73);
	\draw [very thick,blue] (1,1.73) to (0,3.464);
	\draw [very thick,blue] (-2,3.464) to (0,3.464);
	\draw [very thick,blue] (-2,3.464) to (-3,5.20);
	\draw [very thick,blue] (0,3.464) to (1,5.20);
	\draw [very thick,blue] (1,5.20) to (3,5.20);
	\draw [very thick,red] (-1,1.73) to (1,1.73);
	\draw [very thick,red] (-1,1.73) to (-2,3.464);
	\draw [very thick,red] (1,1.73) to (2,3.464);
	\draw [very thick,red] (-2,3.464) to (-1,5.20);
	\draw [very thick,red] (2,3.464) to (1,5.20);
	\draw [very thick,red] (-1,5.20) to (1,5.20);
	\node at (-2.5,6) {\tiny $\vdots$};
	\node at (-1.5,6) {\tiny $\vdots$};
	\node at (-0.5,6) {\tiny $\vdots$};
	\node at (0.5,6) {\tiny $\vdots$};
	\node at (1.5,6) {\tiny $\vdots$};
	\node at (2.5,6) {\tiny $\vdots$};
	\node at (0,1) {\tiny $(0,0)$};
	\node at (0,2.4) {\tiny $(1,1)$};
	\node at (-1,2.75) {\tiny $(0,3)$};
	\node at (1,2.75) {\tiny $(3,0)$};
	\node at (-1,4.1) {\tiny $(1,4)$};
	\node at (1,4.1) {\tiny $(4,1)$};
	\node at (-2,4.46) {\tiny $(0,6)$};
	\node at (2,4.46) {\tiny $(6,0)$};
	\node at (0,4.46) {\tiny $(3,3)$};
	\draw [thick, ->] (1,2.95) to (1,3.9);
	\node at (1.425,3.175) {\tiny $s_{\alpha^{\!\vee}_{\! 0}\!\!, 2}$};
\end{tikzpicture}
};
\endxy
\]
Here we reflect either in a red 
(that is, $\alpha_0=(1,1)$), green 
(that is, $\alpha_1=(2,-1)$) 
or blue (that is, $\alpha_2=(-1,2)$) 
hyperplane, and the
$r$ measures the hyperplane-distance 
from the origin (both indicated in the left picture above). 
In the right picture we have indicated 
the linkage (we have also displayed 
one of the dot-reflections).


Theorem~\ref{thm-link} means now that $T_q((1,1))$ satisfies
\[
(T_q((1,1)):\Dm)\neq 0\quad\Rightarrow\quad\mu\in\{(0,0),(1,1)\}
\]
and $T_q((3,3))$ satisfies
\[
(T_q((3,3)):\Dm)\neq 0\quad\Rightarrow\quad\mu\in\{(0,0),(1,1),(3,0),(0,3),(4,1),(1,4),(3,3)\}.
\]
We calculate the precise values later in Example~\ref{ex-sl3again}.
\end{ex}



In order to get our hands on the multiplicities, we 
need Soergel's version of the \textit{(affine) parabolic Kazhdan-Lusztig polynomials}, 
which we denote by
\begin{equation}\label{eq-kl}
n_{\mu\lambda}(t)\in\Z[v,v^{-1}],\quad \lambda,\mu\in X^+-\rho.
\end{equation}
For brevity, we do not recall the definition of these polynomials (which can 
be computed algorithmically) here, but refer 
to~\cite[Section~3]{soe3} where the relevant polynomial 
is denoted $n_{y,x}$ for $x,y\in W_l$ (which translates by~\eqref{eq-translationweyl} to our notation). 
The main point for us is the following theorem due to Soergel.
\begin{thm}(\textbf{Multiplicity formula})\label{thm-mult}
Suppose $\K=\C$ and $q$ is a complex, primitive $l$-th root of unity.
For each pair $\lambda,\mu\in X^+$ with $\lambda$ being an $l$-regular $\Uq$-weight 
(that is, $\Tl$ belongs to a regular block of $\T$) we have
\[
(\Tl:\Dm)=(\Tl:\Nm)=n_{\mu\lambda}(1).
\]
In particular, if $\lambda,\mu\in X^+$ are not linked, then $n_{\mu\lambda}(v)=0$.\makeqed
\end{thm}
\begin{proof}
This follows from~\cite[Theorem~5.12]{soe4} 
(see also~\cite[Conjecture~7.1]{soe3}).
\end{proof}


\begin{ex}\label{ex-sl3again}
Back to Example~\ref{ex-sl3alcoves}: 
for $\nu=\omega_1+\omega_2=(1,1)$ we have $n_{\nu\nu}(v)=1$ 
and $n_{\nu(0,0)}(v)=v$ as shown in 
the left picture below.
Similarly, for $\xi=3\omega_1+3\omega_2=(3,3)$ the only non-zero 
parabolic Kazhdan-Lusztig polynomials are $n_{\xi\xi}(v)=1$, $n_{\xi(1,4)}(v)=v=n_{\xi(4,1)}(v)$, 
$n_{\xi(0,3)}(v)=v^2=n_{\xi(3,0)}(v)$ and $n_{\xi\nu}(v)=v^3$ 
as illustrated on the right below.
\[
\nu\colon
\xy
(0,0)*{
\begin{tikzpicture}[scale=.75]
	\draw [very thick,green] (0,0) to (-1,1.73);
	\draw [very thick,green] (-1,1.73) to (0,3.464);
	\draw [very thick,green] (0,3.464) to (2,3.464);
	\draw [very thick,green] (0,3.464) to (-1,5.20);
	\draw [very thick,green] (2,3.464) to (3,5.20);
	\draw [very thick,green] (-3,5.20) to (-1,5.20);
	\draw [very thick,blue] (0,0) to (1,1.73);
	\draw [very thick,blue] (1,1.73) to (0,3.464);
	\draw [very thick,blue] (-2,3.464) to (0,3.464);
	\draw [very thick,blue] (-2,3.464) to (-3,5.20);
	\draw [very thick,blue] (0,3.464) to (1,5.20);
	\draw [very thick,blue] (1,5.20) to (3,5.20);
	\draw [very thick,red] (-1,1.73) to (1,1.73);
	\draw [very thick,red] (-1,1.73) to (-2,3.464);
	\draw [very thick,red] (1,1.73) to (2,3.464);
	\draw [very thick,red] (-2,3.464) to (-1,5.20);
	\draw [very thick,red] (2,3.464) to (1,5.20);
	\draw [very thick,red] (-1,5.20) to (1,5.20);
	\node at (-2.5,6) {\tiny $\vdots$};
	\node at (-1.5,6) {\tiny $\vdots$};
	\node at (-0.5,6) {\tiny $\vdots$};
	\node at (0.5,6) {\tiny $\vdots$};
	\node at (1.5,6) {\tiny $\vdots$};
	\node at (2.5,6) {\tiny $\vdots$};
	\node at (0,1) {\tiny $v$};
	\node at (0,2.4) {\tiny $1$};
\end{tikzpicture}
};
\endxy\quad\quad
\xi\colon
\xy
(0,0)*{
\begin{tikzpicture}[scale=.75]
	\draw [very thick,green] (0,0) to (-1,1.73);
	\draw [very thick,green] (-1,1.73) to (0,3.464);
	\draw [very thick,green] (0,3.464) to (2,3.464);
	\draw [very thick,green] (0,3.464) to (-1,5.20);
	\draw [very thick,green] (2,3.464) to (3,5.20);
	\draw [very thick,green] (-3,5.20) to (-1,5.20);
	\draw [very thick,blue] (0,0) to (1,1.73);
	\draw [very thick,blue] (1,1.73) to (0,3.464);
	\draw [very thick,blue] (-2,3.464) to (0,3.464);
	\draw [very thick,blue] (-2,3.464) to (-3,5.20);
	\draw [very thick,blue] (0,3.464) to (1,5.20);
	\draw [very thick,blue] (1,5.20) to (3,5.20);
	\draw [very thick,red] (-1,1.73) to (1,1.73);
	\draw [very thick,red] (-1,1.73) to (-2,3.464);
	\draw [very thick,red] (1,1.73) to (2,3.464);
	\draw [very thick,red] (-2,3.464) to (-1,5.20);
	\draw [very thick,red] (2,3.464) to (1,5.20);
	\draw [very thick,red] (-1,5.20) to (1,5.20);
	\node at (-2.5,6) {\tiny $\vdots$};
	\node at (-1.5,6) {\tiny $\vdots$};
	\node at (-0.5,6) {\tiny $\vdots$};
	\node at (0.5,6) {\tiny $\vdots$};
	\node at (1.5,6) {\tiny $\vdots$};
	\node at (2.5,6) {\tiny $\vdots$};
	\node at (0,2.4) {\tiny $v^3$};
	\node at (-1,2.75) {\tiny $v^2$};
	\node at (1,2.75) {\tiny $v^2$};
	\node at (-1,4.1) {\tiny $v$};
	\node at (1,4.1) {\tiny $v$};
	\node at (0,4.46) {\tiny $1$};
\end{tikzpicture}
};
\endxy
\]
Therefore, we have, by Theorem~\ref{thm-mult}, that $(T_q(\nu):\Dm)=1$ if $\mu\in\{(0,0),(1,1)\}$ and 
$(T_q(\nu):\Dm)=0$ if $\mu\notin\{(0,0),(1,1)\}$. 
We encourage the reader to work out $(T_q(\xi):\Dm)$ 
by using the above patterns and Example~\ref{ex-sl3alcoves}.
For all patterns in rank $2$ see~\cite{sdiplom}.
\end{ex}


\begin{rem}\label{rem-walls}
Assume $\lambda\in X^+$ to be not $l$-regular. Set 
$W_{\lambda}=\{w\in W_l\mid w.\lambda=\lambda\}$.
Then we can find a unique 
$l$-regular $\overline{\lambda}\in W_l.0$ such 
that $\lambda$ is in the closure of the alcove containing 
$\overline{\lambda}$ and $\overline{\lambda}$ is maximal in $W_{\lambda}.\overline{\lambda}$.
Examples for $\fg=\sll{2}$ and $\fg=\sll{3}$ are
\[
\xy
(0,0)*{
\begin{tikzpicture}[scale=.75]
	\draw [very thick, directed=0.95] (3,0) to (4.5,0);
    \node at (-1.5,0) {\tiny $\cdots$};
	\node[red] at (0,0) {\tiny $\bullet$};
	\node[green] at (3,0) {\tiny $\bullet$};
	\node[red] at (6,0) {\tiny $\bullet$};
	\node at (7.5,0) {\tiny $\cdots$};
	\node at (3,0.25) {\tiny $\lambda$};
	\node at (4.5,0) {\tiny $\bullet$};
	\node at (4.5,0.25) {\tiny $\overline{\lambda}$};
	\end{tikzpicture}
};
\endxy
\quad\text{and}\quad
\xy
(0,0)*{
\begin{tikzpicture}[scale=.75]
	\draw [very thick,blue] (0,0) to (-1,1.73);
	\draw [very thick,blue] (-1,1.73) to (0,3.464);
	\draw [very thick,blue] (0,3.464) to (2,3.464);
	\draw [very thick,blue] (0,3.464) to (-1,5.20);
	\draw [very thick,blue] (2,3.464) to (3,5.20);
	\draw [very thick,blue] (-3,5.20) to (-1,5.20);
	\draw [very thick,green] (0,0) to (1,1.73);
	\draw [very thick,green] (1,1.73) to (0,3.464);
	\draw [very thick,green] (-2,3.464) to (0,3.464);
	\draw [very thick,green] (-2,3.464) to (-3,5.20);
	\draw [very thick,green] (0,3.464) to (1,5.20);
	\draw [very thick,green] (1,5.20) to (3,5.20);
	\draw [very thick,red] (-1,1.73) to (1,1.73);
	\draw [very thick,red] (-1,1.73) to (-2,3.464);
	\draw [very thick,red] (1,1.73) to (2,3.464);
	\draw [very thick,red] (-2,3.464) to (-1,5.20);
	\draw [very thick,red] (2,3.464) to (1,5.20);
	\draw [very thick,red] (-1,5.20) to (1,5.20);
	\draw [thick,directed=.9] (0,3.43) to (0,4.46);
	\draw [thick,directed=.9] (1.45,4.3) to (2,4.6);
	\draw [thick,directed=.9] (1.52,2.65) to (0.97,2.95);
	\node at (-2.5,6) {\tiny $\vdots$};
	\node at (-1.5,6) {\tiny $\vdots$};
	\node at (-0.5,6) {\tiny $\vdots$};
	\node at (0.5,6) {\tiny $\vdots$};
	\node at (1.5,6) {\tiny $\vdots$};
	\node at (2.5,6) {\tiny $\vdots$};
	\node at (2,4.575) {\tiny $\bullet$};
	\node at (2.2,4.65) {\tiny $\overline{\lambda}$};
	\node at (1.5,4.30) {\tiny $\bullet$};
	\node at (1.55,4.05) {\tiny $\lambda$};
	\node at (1,2.925) {\tiny $\bullet$};
	\node at (0.8,3) {\tiny $\overline{\mu}$};
	\node at (1.52,2.63) {\tiny $\bullet$};
	\node at (1.55,2.4) {\tiny $\mu$};
	\node at (0,4.46) {\tiny $\bullet$};
	\node at (0,4.7) {\tiny $\overline{\nu}$};
	\node at (0,3.43) {\tiny $\bullet$};
	\node at (0.25,3.3) {\tiny $\nu$};
	\node at (0,1) {\tiny $0$};
\end{tikzpicture}
};
\endxy
\]
Assume now that $\lambda,\mu\in X^+$ are linked. Then
\begin{equation}\label{eq-translation}
(\Tl:\Delta_q(\mu))=(T_q(\overline{\lambda}):\Delta_q(\overline{\mu}))
\end{equation}
and the latter is given by Theorem~\ref{thm-mult}. 
Compare to~\cite[Proposition~5.2 and Corollary~5.4]{an3}. 
The proof of~\eqref{eq-translation} 
follows by using arguments involving translation functors. For brevity, we 
discuss the details only in~\cite{astproofs}.
\end{rem}



Since the polynomials from~\eqref{eq-kl} can be computed inductively, we can use 
Theorem~\ref{thm-mult} and Remark~\ref{rem-walls} in the case $\K=\C$ 
to \textit{explicitly} calculate the 
decomposition of a tensor product of $\Uq$-tilting modules 
$T=T_q(\lambda_1)\otimes\dots\otimes T_q(\lambda_d)$ into its indecomposable summands:
\begin{itemize}
\item Calculate, by using Theorem~\ref{thm-mult} and Remark~\ref{rem-walls}, 
$(T_q(\lambda_i):\Dm)$ for $i=1,\dots,d$.
\item This gives the multiplicities of $T$, by the Corollary~\ref{cor-grothen} and the fact that 
$\chi(\Dl)$ are as in the classical case.
\item Use~\eqref{eq-grgr} to recursively compute the decomposition of $T$ (starting with 
any maximal $\Uq$-weight of $T$).
\end{itemize}


\begin{ex}\label{ex-sl2again}
Let us come back to our favourite case, that is, $\fg=\sll{2}$, $\K=\C$ and $l=3$.
In the regular cases we have $T_q(k)\cong \Delta_q(k)$ for $k=0,1$ and the parabolic Kazhdan-Lusztig 
polynomials are
\[
n_{jk}(v)=\begin{cases}1,&\text{if }j=k,\\
v,&\text{if }j<k\text{ are separated by precisely one wall},\\
0,&\text{else},\end{cases}
\]
for $k>1$. By~\eqref{eq-translation} we obtain $T_q(k)\cong \Delta_q(k)$ for $k\in\N$ singular, hence, 
the two singular blocks $\T_{-1}$ and $\T_2$ are semi-simple.


In Example~\ref{ex-sl2c} we have already calculated 
$T_q(1)\otimes T_q(1)\cong T_q(2)\oplus T_q(0)$.
Let us go one step further now:
$T_q(1)\otimes T_q(1)\otimes T_q(1)$ has only 
$(T_q(1)^{\otimes 3}:\Delta_q(3))=1$ and 
$(T_q(1)^{\otimes 3}:\Delta_q(1))=2$ as non-zero multiplicities.
This means that $T_q(3)$ is a summand of $T_q(1)\otimes T_q(1)\otimes T_q(1)$. Since 
$T_q(3)$ has only 
$(T_q(3):\Delta_q(3))=1$ and $(T_q(3):\Delta_q(1))=1$ as non-zero 
multiplicities (by the calculation of the periodic Kazhdan-Lusztig polynomials), we have
\begin{equation}\label{eq-decom1}
T_q(1)\otimes T_q(1)\otimes T_q(1)\cong T_q(3)\oplus T_q(1)\in\T_1.
\end{equation}
Moreover, we have (as we, as usual, encourage the reader to work out)
\[
T_q(1)\otimes T_q(1)\otimes T_q(1)\otimes T_q(1)\cong (T_q(4)\oplus T_q(0))\oplus (T_q(2)\oplus T_q(2)\oplus T_q(2))\in \T_0\oplus\T_2.
\]


To illustrate how this decomposition depends on $l$: assume now that $l>3$. 
Then, which can be verified similarly as in Example~\ref{ex-alcove}, the $\Uq$-tilting module
$T_q(3)$ is in the fundamental alcove $\cal{A}_0$. 
Thus, by Theorem~\ref{thm-link}, $T_q(3)$ is simple as in the ``classical'' case. Said otherwise, 
we have $T_q(3)\cong \Delta_q(3)$. 
Hence, in the same spirit as above, we obtain (as in the generic case)
\begin{equation}\label{eq-decom2}
T_q(1)\otimes T_q(1)\otimes T_q(1)\cong T_q(3)\oplus (T_q(1)\oplus T_q(1))\in\T_3\oplus\T_1
\end{equation}
in contrast to the decomposition in~\eqref{eq-decom1}.
\end{ex}
